High precision meteor observations with the Canadian Automated Meteor Observatory -- Data reduction pipeline and application to meteoroid mechanical strength measurements

Context. The mirror tracking system of the Canadian Automated Meteor Observatory (CAMO) can track meteors in real time, providing an effective angular resolution of 1 arc second and a temporal resolution of 100 frames per second. Aims. We describe the upgraded hardware and give details of the data calibration and reduction pipeline. We investigate the influence of meteor morphology on radiant and velocity measurement precision, and use direct observations of meteoroid fragmentation to constrain their compressive strengths. Methods. On July 21, 2017, CAMO observed a ~4 second meteor on a JFC orbit. It had a shallow entry angle ~8 deg and 12 fragments were visible in the narrow-field video. The event was manually reduced and the exact moment of fragmentation was determined. The aerodynamic ram pressure at the moment of fragmentation was used as a proxy for compressive strength, and strengths of an additional 19 fragmenting meteoroids were measured in the same way. The uncertainty in the atmosphere mass density was estimated to be +/-25% using NAVGEM-HA data. Results. We find that meteor trajectory accuracy significantly depends on meteor morphology. The CAMO radiant and initial velocity precision for non-fragmenting meteors with short wakes is ~0.5' and 1 m/s, while that for meteors with fragments or long wakes is similar to non-tracking, moderate field of view optical systems (5', ~50 m/s). Measured compressive strengths of 20 fragmenting meteoroids (with less precise radiants due to their morphology) was in the range of 1-4 kPa, which is in excellent accord with Rosetta in-situ measurements of 67P. Fragmentation type and strength do not appear to be dependent on orbit. The mass index of the 12 fragments in the July 21 meteoroid was very high (s = 2.8), indicating possible progressive fragmentation.

==> extras.tex <==
\subsection{Calibration plates}

Four distinct calibration plates are used operationally, and for data reduction. The \textit{calib} plate is the standard astrometric plate used for the wide-field camera, while the \textit{guide} plate is used for pointing the mirrors to any corresponding position on the wide-field image. The \textit{scale} and the \textit{exact} plate are used for obtaining high-precision measurements of meteor positions on narrow-field images. The description of each plate is given below, and a summary is given in Table \ref{tab:plates}.
    
\subsubsection{calib plate}
The \textit{calib} plate is a standard calibration plate which maps image pixel coordinate of the wide-field camera ($w_x$, $w_y$) to horizontal celestial coordinates ($\theta$, $\varphi$). The AST plate format is used for this purpose. The \textit{calib} plate can be made using METAL, whereby the user manually matches the stars on the image with the stars in the catalog until a satisfactory calibration is achieved, as described in \cite{weryk2012simultaneous}, section 3.3.


\subsubsection{guide plate}
When a meteor is detected on the wide-field system, the mirrors need to be steered to track it. For that purpose, the \textit{guide} plate is used. This plate maps image coordinates of the wide-field camera ($w_x$, $w_y$) to mirror encoder coordinates ($h_x$, $h_y$). As both coordinates are planar, the AFF plate format is used. This plate can be generated using the \textit{mosaic} program, which incrementally moves the mirrors across the sky and takes snapshots using the narrow-field camera to generate a mosaic image. The stars on this composite image are located and paired with the stars on the wide-field image to find the fit parameters. A more detailed description was given in \cite{weryk2013camo}, section 3.4. Another way of creating \textit{guide} plates is using the \textit{mircal} program, which uses data collected by \textit{mirchk}.


\subsubsection{scale plate}
For every video frame, the current mirror encoder position ($h_x$, $h_y$) corresponds to the centre of the narrow-field image ($n_x = 320$, $n_y = 240$). If one wants to convert the position of an object in the narrow-field image to celestial coordinates ($\theta$, $\varphi$), one first needs to find its position in mirror encoder coordinates (as outlined in the beginning of section \ref{section:data_calibration}), and use the \textit{exact} plate to convert them to ($\theta$, $\varphi$).

The \textit{scale} plate is used to convert the offsets from the centre of the narrow-field image ($\Delta n_x$, $\Delta n_y$) to the corresponding offsets in mirror encoder coordinates ($\Delta h_x$, $\Delta h_y$) and is implemented as an AFF plate. The plate should be stable against pointing changes, and it is only dependent on the optical setup and alignment. An initial version of the plate can be created with \textit{mosaic}, but a more accurate version can be created with \textit{mircal} and \textit{mirchk} (see section \ref{section: mirchk}).


\subsubsection{exact plate}

The \textit{exact} plate directly maps the mirror encoder coordinates ($h_x$, $h_y$) to the celestial horizontal coordinates ($\theta$, $\varphi$) and it is implemented as an AST plate. Paired with the \textit{scale} plate, this plate allows for high-precision trajectory estimation from measurements on narrow-field images. This plate is created using \textit{mircal} and \textit{mirchk}.

Before the \textit{exact} plate was introduced, narrow-field events were reduced by combining the \textit{guide} plate with the \textit{calib} plate, which was refered to as a ``boot-strapped'' fit. This effectively limited the measurement accuracy to the accuracy of astrometric calibration of the wide-field camera.


% Ablation modelling
% - In Vida et al. 2018 we showed that initial velocity accuracy is driven by the amount of deceleration a meteoroid experienced before becoming visible. This deceleration can be up to 750 m/s and depends on meteoroid mass and physical properties (bulk density, ablation coefficient).
% No one was able to systematically fit wakes

%   - Skipping the first few frames until the mirrors settle (show figure)

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % OLD TEXT BELOW
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newpage

% \subsection{Calibration software}
% \subsubsection{Mirchk} \label{section: mirchk}
% The most important step in the calibration is pairing the mirror encoder coordinates to celestial coordinates. Every 2 hours the system stops tracking meteors and runs \textit{mirchk}, which collects the positions of 80 stars by steering the mirrors on their predicted coordinates and finds their actual positions. With this data, one can fit the fit parameters which describe the transformation from mirror encoder units to celestial coordinates. Initially, the steering was done by using an operational \textit{guide} plate - the stars were located on the wide-field image and mirrors were steered on their approximate position. The position was refined by moving the brightest star in the field of view to the centre of the image, thus matching the mirror encoder positions ($h_x$, $h_y$), assumed to correspond to the centre of the narrow-field image, to ($\theta$, $\varphi$) of the star. An operational \textit{scale} plate is used for calculating the offset in mirror encoder units needed to centre the star. Figure \ref{fig:mirchk_star_centring} shows a star before and after centring. As it can be noticed, after centring, the star is not right in the centre of the image due to the imperfection of the operational \textit{scale} plate. Nevertheless, the information for creating a calibration \textit{scale} plate are obtained. During the data calibration procedure, each star is ``virtually'' centred using the calibration \textit{scale} plate before creating the calibration \textit{exact} plate.

% \begin{figure}
%   \includegraphics[width=\linewidth]{media/mirchk_star_centring.png}
%   \caption{The left inset shows the position of the star after pointing to it using the operational \textit{exact} plate. The right inset shows the position of the star after centring. The white cross in the middle of both insets marks the centre of the image.}
%   \label{fig:mirchk_star_centring}
% \end{figure}

% The downside of using a \textit{guide} plate to steer the mirrors was that the field of view covered by the mirrors is about twice the field of view of the wide-field camera, thus leaving some parts of the mirror encoder coordinate phase space not covered by the calibration. This problem was solved by using an operational \textit{exact} plate which can directly reverse map celestial coordinates of stars to mirror encoder positions. Understandably, this operational \textit{exact} plate is only valid if nothing is physically changed in the system. If the location or the orientation of the galvanometers were to change, one would need to revert to an operational \textit{guide} plate and only then obtain a new operational \textit{exact} plate. The operational \textit{exact} plate is only precise enough to locate the star within the field of view of the narrow-field camera, while a special \textit{exact} plate is made every night for data calibration purposes. Furthermore, a filtered version of the SKY2000 catalogue is used for looking up the stars - all stars closer than $0.5\degree$ to each other, and if their magnitudes differed less than 1 magnitude, were removed from the catalog. This was done to prevent the system from locking on to the wrong star during the calibration procedure.

% The other function of \textit{mirchk} is to collect data for fitting a \textit{scale} plate. Every time a star is centered, \textit{mirchk} collects the initial image coordinates of the star, the coordinates of the star after centring (which may not be perfectly in the centre of the image, because the the operational \textit{scale} plate may not be perfect as well), and finally the value of ($\Delta h_x$, $\Delta h_y$) by which the mirrors were moved. From the difference in the two image positions of the star, one can calculate ($\Delta n_x$, $\Delta n_y$) and fit the \textit{scale} plate which can be used for calibration. Nevertheless, a problem might arise if the operational \textit{exact} plate shows a systematic offset, or if it is too good. To illustrate - if the operational \textit{exact} plate always puts a star a bit up and left of the image centre, and the centring algorithms centres the star, the resulting \textit{scale} plate will only be good for calculating positions which are in the upper left quadrant of the image because there was no information how to centre an object in any other part of the image. Moreover, the operational \textit{exact} plate initially positions the star very close to the image centre, the resulting \textit{scale} plate will not be good for positions far from the centre of the image. For those reasons, a special calibration procedure is preformed to move the mirrors in such a way to optimally cover the ($\Delta n_x$, $\Delta n_y$) phase space. Figure \ref{fig:scale_phase_space_hexagon} shows one of four patterns performed by the mirrors which result in 6 points in the ($\Delta n_x$, $\Delta n_y$) phase space, distributed as a hexagon. A randomness of $\pm 25$ pixels in each position is intentionally introduced to avoid having multiple points in the phase space at the same place.

% \subsubsection{Mircal}
% software for creating all 4 types of plates. It uses data files produced by mirchk.

%      \begin{enumerate}
%         \item Levenberg-Marquardt method is used for fitting the plates
%         \item The fits are inspected manually – the software lists all stars and their residuals from the fit. As there is a possibility there are some outliers in the data, they can be manually removed by specifying ordinal numbers of stars with high residuals.
%         \item To preform data reduction of CAMO data, one needs 2 plates: a scale and an exact plate
%      \end{enumerate}




% \section{Data reduction}

% \subsection{Preparation}
    
% To streamline the data reduction process, a Python script was developed which automatically collects all necessary data files (video files of the event, star files needed to do the calibrations), organizes the files properly, generates scale and exact plates using mircal. The outliers in the star data are rejected automatically – the algorithm works iteratively by finding which star should be rejected to obtain the largest reduction in average fit residuals; stopping upon reaching a predefined average residual threshold.


% \subsection{Data description}

% \begin{enumerate}
%     \item Vid files – raw 640x480 video frames stored in a binary format
%     \item ev*.txt files – info correlating individual frames to mirror coordinates of the FOV centre
% \end{enumerate}


% \subsection{Mirfit}
% Mirfit – integrated solution for astrometry, photometry, deceleration modelling and orbit determination
% \begin{enumerate}
%     \item Calibration files are loaded (exact and scale plate)
%     \begin{enumerate}
%         \item Exact – transforms mirror coordinates (Hx, Hy) to sky coordinates (azimuth, zenithal distance)
%         \item Scale – transforms image coordinates to differences in mirror coordinates from the image centre
%     \end{enumerate}
%     \item Deciding where to do the picks - settled on centroiding. Show a sequance of 3D (X, Y, intensity) plots to show the central peak, which is not Gaussian.
%     \item Astrometry picks are manually done by selecting a general ROI around the body of the meteor (follow this up with some figures and examples). Centroiding is preformed on pixels within this circular ROI. Describe the whole path from image coordinate to (theta, phi): (x, y) –(scale)$\rightarrow$ (hu, hv) + (hx, hy) from interpolated mirror positions –(exact)$\rightarrow$ (theta, phi)
%     \item Mirfit photometry?
% \end{enumerate}


% \section{Ablation modelling and initial velocity estimation}

% After trajectory estimation, the question was how to properly estimate the uncertainties in the initial velocity, and what is the real pre-atmosphere velocity. The downside of measurements from CAMO narrow-field is that they only begin after the ablation and light production had started, the meteor had been detected on the wide-field camera, the tracking parameters had been calculated from the first 4 video frames and the mirrors were steered to track the meteor. This whole procedure may take \SI{50}{\milli \s} or longer, while the meteor is ablating the decelerating. If one was to blindly calculate the initial velocities on this data, they would surely be underestimated. Furthermore, a couple of frames is needed for the mirrors to settle after the tracking has started, which may introduce additional uncertainty in the initial velocity. Figure \ref{fig:mirror_wobble} shows the wobble of the mirrors on one of the first video frames after the tracking has started - note the two background stars. The wobble disappears after several frames and its amplitude is dependant on how far the pre-tracking position of the mirrors was (when they were idle waiting for an event) from the tracked trajectory.
% To estimate the velocity of meteoroids before entering the atmosphere, we are using meteor ablation model by \cite{campbell2004model}.


% \begin{figure}
%   \includegraphics[width=\linewidth]{media/mirror_wobble.png}
%   \caption{Left: One of the first narrow-field video frames after the tracking has started. Two stars can be seen at the right side of the figure as L shaped curves. Due to the mirror wobble and the ongoing fragmentation of the meteor, it is difficult to make consistent position measurements. Right: The wobble stops after several frames.}
%   \label{fig:mirror_wobble}
% \end{figure}


% \begin{enumerate}
%     \item Initial mass estimate from widefield photometry (this limits the used trail length to the part within the wide FOV). The magnitudes are interpolated with spline interpolation and integrated to obtain the intensity. 
    
%     \begin{equation}
%         I(t) = P_{0m} 10^{-0.4 M(t)}
%     \end{equation}
    
%     \begin{equation}
%         m = \frac{2}{\tau v_{avg}^2} \int_{0}^{t_{max}} I(t) dt
%     \end{equation}
    
%     Used $\tau = 0.07\%$, plus minus order of magnitude (give the equation for the mass). Cite various sources for luminous efficiency, and cite Dilini's paper. The number $P_{0m} = 840W$ is the power output for a zero absolute magnitude meteor in the R bandpass (we are using stars in the R band for photometry), for T = 4500K \citep{weryk2013simultaneous}.
%     \item Inverse single-body meteor ablation modelling using \cite{campbell2004model} model, range of parameters from \cite{kikwaya2011bulk}, minimizing the difference in meteor length along the trail. Only the first 25\% of the meteor trajectory is fitted (or at least 4 points) - the fragmentation would a large influence on the fit if we took later parts. Only those solutions which are within the measurement precision (defines as the geometrical mean of the along-track RMS and perpendicular to the track RMS). We have determined that density has the largest influence on the result, while other parameters are negligible influence (because we are only looking fitting the first part of the trajectory, where the effects which are using those parameters are minimal).
%     \item Vinf (@180 km) estimate from modelling – comparison to the geometrical solution. In many cases the geometrically estimated Vinf is not at the centre of the modelled velocity at 180km range due to two causes:
%     \begin{enumerate}
%         \item If the initial part of the trajectory was recorded at the beginning of the ablation - the velocity at 180 km is lower than the initial velocity because of gravitational acceleration.
%         \item If the initial part of the trajectory was recorded well into the ablation - the velocity at 180 km is higher because it is the velocity before atmospheric deceleration.
%     \end{enumerate}
%     \item Uncertainties are calculated from the angular residuals in the fit - the $(\theta, \varphi)$ of initial points are Monte Carlo drawn from $\theta_i = \mathcal{N} \left(\theta_i, \sigma_{\theta} \right)$, $\varphi_i = \mathcal{N} \left(\varphi_i, \sigma_{\varphi} \right)$ so that every measurement point is sampled 10 times.
%     \item Orbits calculated using a combination of \cite{ceplecha1987geometric}, \cite{clark2010searching}, and \cite{jenniskens2011cams} method (best of all worlds) - the Earth's position is calculated using JPL DE430 ephemerids \citep{folkner2014planetary}
% \end{enumerate}
